Flight Time Improvement Using Adaptive Model Predictive Control for Unmanned Aerial Vehicles

Intelligent aerial platforms such as Unmanned Aerial Vehicles (UAVs) are expected to revolutionize various fields, including transportation, traffic management, field monitoring, industrial production, and agricultural management. Among these, precise control is a critical task that determines the performance and capabilities of UAV systems. However, current research primarily focuses on trajectory tracking and minimizing flight errors, with limited attention to improving flight time. In this paper, we propose a Model Predictive Control (MPC) approach aimed at minimizing flight time while addressing the limitations of the commonly used classical MPC controllers. Furthermore, the MPC method and its application for UAV control are presented in detail. Finally, the results demonstrate that the proposed controller outperforms the standard MPC in terms of efficiency. Moreover, this approach shows potential to become a foundation for integrating intelligent algorithms into basic controllers.

==> vncaps.tex <==
% Copyright 2000-2006 Werner Lemberg <wl@gnu.org> and
%                     Han The Thanh <hanthethanh@gmx.net>.
% This file is part of vntex.  License: LPPL, version 1.3 or newer,
% according to http://www.latex-project.org/lppl.txt

\ifx\ProvidesFile\undefined \else
  \ProvidesFile{vncaps.tex}[2006/06/07 v1.1 Captions in Vietnamese]  
\fi
 
% Vietnamese captions; edit them in viscii/tcvn/utf8, then use
% `vntovn viscii vntex' or a similar command to convert to vntex.
%
% History
%
% ????/??/??:
%     Split off captions from vietnam.ldf.
%     Add \captionsenglish, \dateUSenglish, and \dateenglish.
%
% 2005/04/21:
%     Add copyright message.
%     Don't use `{}' but a space after macros which don't have arguments.
%
% 2006/06/07:
%     Fix bug in \indexname.  Add version number.

\ifx\providecommand \undefined
  \let\providecommand \def
\fi

\providecommand\captionsvietnam{% 
  \def\prefacename{L\`\ohorn i n\'oi \dj\`\acircumflex u}%
%  \def\refname{T\`ai li\d\ecircumflex u}%
  \def\Acknowledgmentname{L\`\ohorn i c\h{a}m \ohorn n}%
  \def\refname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
%  \def\abstractname{T\'om t\'\abreve t n\d\ocircumflex i dung}
  \def\abstractname{T\'om t\'\abreve t}
  \def\IEEEkeywordsname{T\`\uhorn \, kh\'oa}
  \def\bibname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
  \def\chaptername{Ch\uhorn \ohorn ng}%
  \def\appendixname{Ph\d{u} l\d{u}c}%
  \def\contentsname{M\d{u}c l\d{u}c}%
  \def\listfigurename{Danh s\'ach h\`inh v\~e}%
  \def\listtablename{Danh s\'ach b\h{a}ng}%
  \def\indexname{Ch\h{i} m\d{u}c}% 
  \def\figurename{H\`inh}%
  \def\tablename{B\h{a}ng}%
  \def\partname{Ph\`\acircumflex n}%
  \def\pagename{Trang}%
  \def\headpagename{Trang}%
  \def\seename{Xem}%
  \def\alsoname{Xem th\ecircumflex m}%
  \def\enclname{K\`em theo}%
  \def\ccname{C\`ung g\h\uhorn i}%
  \def\headtoname{G\h\uhorn i}%
  \def\proofname{Ch\'\uhorn ng minh}}

\providecommand\datevietnam{%
  \def\today{%
    Ng\`ay \number\day\space
    th\'ang \number\month\space
    n\abreve m \number\year}}

\providecommand\captionsenglish{%
  \def\prefacename{Preface}%
  \def\refname{References}%
  \def\abstractname{Abstract}%
  \def\bibname{Bibliography}%
  \def\chaptername{Chapter}%
  \def\appendixname{Appendix}%
  \def\contentsname{Contents}%
  \def\listfigurename{List of Figures}%
  \def\listtablename{List of Tables}%
  \def\indexname{Index}%
  \def\figurename{Figure}%
  \def\tablename{Table}%
  \def\partname{Part}%
  \def\enclname{encl}%
  \def\ccname{cc}%
  \def\headtoname{To}%
  \def\pagename{Page}%
  \def\headpagename{Page}%
  \def\prefacename{Preface}%
  \def\seename{see}%
  \def\alsoname{see also}}

\providecommand\dateenglish{%
  \def\today{%
    \ifcase\day\or 1st\or 2nd\or 3rd\or 4th\or 5th\or 6th\or 7th\or
    8th\or 9th\or 10th\or 11th\or 12th\or 13th\or 14th\or 15th\or
    16th\or 17th\or 18th\or 19th\or 20th\or 21st\or 22nd\or 23rd\or
    24th\or 25th\or 26th\or 27th\or 28th\or 29th\or 30th\or 31st\fi
    ~\ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space
    \number\year}}

\providecommand\dateUSenglish{%
  \def\today{%
    \ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space\number\day, \number\year}}

\endinput

% end of vncaps.tex

